Independent measurement of the Hoyle state $\beta$ feeding from 12B using Gammasphere

Using an array of high-purity Compton-suppressed germanium detectors, we performed an independent measurement of the $\beta$-decay branching ratio from $^{12}\mathrm{B}$ to the second-excited (Hoyle) state in $^{12}\mathrm{C}$. Our result is $0.64(11)\%$, which is a factor $\sim 2$ smaller than the previously established literature value, but is in agreement with another recent measurement. This could indicate that the Hoyle state is more clustered than previously believed. The angular correlation of the Hoyle state $\gamma$ cascade has also been measured for the first time. It is consistent with theoretical predictions.

==> plots/decay_scheme/simplified.tex <==
\newcommand{\tsize}{}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\tbf}[1]{\textbf{#1}}

\newcommand{\lwidth}{7em}
\newcommand{\sgap}{5em}
\newcommand{\agap}{0.5em}


\begin{tikzpicture}[line width=0.8mm, text=black, draw=black, font=\boldmath
]

	% Box (resonances in 12C)
	% \draw[draw,line width=75pt,-,black!30] (15em,3.88cm) -- (22em,3.88cm);	   

	% Gamma decay
	\draw[->,line width=0.06cm] (1.5*\lwidth+\sgap,1.4cm) -- ++(0,-1.3cm) node[pos=0.5,left]{\tsize $\mbf{\gamma}$};		
        \draw[->,line width=0.06cm] (1.5*\lwidth+\sgap,1.4cm) -- ++(0,-1.3cm) node[pos=0.5,right]{\tsize $4.439$};		

	\draw[->,line width=0.06cm] (1.5*\lwidth+\sgap,2.5cm) -- ++(0,-0.9cm) node[pos=0.4,left]{\tsize $\mbf{\gamma}$};		
	\draw[->,line width=0.06cm] (1.5*\lwidth+\sgap,2.5cm) -- ++(0,-0.9cm) node[pos=0.4,right]{\tsize $3.215$};		
        
	% 3-alpha threshold
	\draw[-] (2*\lwidth+2*\sgap,2.43cm) -- ++(\lwidth,0) node[pos=0.2,above]{\tsize{\tbf{7.27}}} node[pos=0.5,below]{ \tsize $\mbf{\alpha+\alpha+\alpha}$}; 
	\draw[-,dashed] (0em, 2.43cm) -- ++(2*\sgap+3*\lwidth, 0);	

	% p+11B	
	\draw[-] (0em,4.45cm) -- ++(\lwidth,0) node[pos=0.2,above]{\tsize \tbf{13.37}}node[pos=0.5,below]{ \tsize $\mbf{^{12}}$\tbf{B}}; 	
        \draw[->,line width=0.06cm] (\lwidth+\agap, 4.3cm) -- (\lwidth+\sgap-\agap, 2.6cm) node[pos=0.5, above=0.4cm]{\tsize$\beta^{-}$};
	\draw[->,line width=0.06cm] (\lwidth+\agap, 4.3cm) -- (\lwidth+\sgap-\agap, 1.7cm);
        \draw[->,line width=0.06cm] (\lwidth+\agap, 4.3cm) -- (\lwidth+\sgap-\agap, 0.2cm);

	% 12C bound states
      	\draw[-] (\lwidth+\sgap, 0.00cm) -- ++(\lwidth,0) node[pos=0.18,above]{\tsize{\tbf{g.s.}}} node[pos=0.92,above]{ \tsize $\mbf{0^+}$} node[pos=0.5,below]{ \tsize $^{12}$\tbf{C}};
      	\draw[-] (\lwidth+\sgap, 1.48cm) -- ++(\lwidth,0) node[pos=0.18,above]{\tsize{\tbf{4.439}}} node[pos=0.92,above]{ \tsize $\mbf{2^+}$};
        \draw[-] (\lwidth+\sgap, 2.55cm) -- ++(\lwidth,0) node[pos=0.18,above]{\tsize{\tbf{7.654}}} node[pos=0.92,above]{ \tsize $\mbf{0^+}$};


\end{tikzpicture}

